Clustering as an Evaluation Protocol for Knowledge Embedding Representation of Categorised Multi-relational Data in the Clinical Domain

Learning knowledge representation is an increasingly important technology applicable in many domain-specific machine learning problems. We discuss the effectiveness of traditional Link Prediction or Knowledge Graph Completion evaluation protocol when embedding knowledge representation for categorised multi-relational data in the clinical domain. Link prediction uses to split the data into training and evaluation subsets, leading to loss of information along training and harming the knowledge representation model accuracy. We propose a Clustering Evaluation Protocol as a replacement alternative to the traditionally used evaluation tasks. We used embedding models trained by a knowledge embedding approach which has been evaluated with clinical datasets. Experimental results with Pearson and Spearman correlations show strong evidence that the novel proposed evaluation protocol is pottentially able to replace link prediction.

==> CLUST-99-Drafts.tex <==
% =================================================
\section{Drafts}
% =================================================
In clinical domain, there are multiple knowledge bases available. By using blockchain technology, people can obtain more information available for data analysis while ensuring the security of personal data.\cite{Panesar2019} The increasing number of multi-relational data also mean that the evaluation of model needs to be carefully considered as a wide range of model applications have higher requirements for model evaluation, especially in the field related to people's health.

Problem Description

The evaluation of embedding process is depending on the link prediction task which need the training and testing process.The link prediction task is focus on the prediction of missing head entity or tail entity in $(h, r, t)$ and it including two metrics: mean rank and hits@n. In this project, we focus on the part of replace tail entity only.To calculate the mean rank, we replace the real tail entity for each triple (h, r, t) in the test set with all the entities in the dictionary and we can obtain fake triples. Then we calculate the score by the function fr(h,t) in order to get all the potential tail we could expect from the all the fake triples. Through this way, we can get a series of scores and then sort the scores in ascending order. 
During this process, we lose the precious information because only part of the data is used to test only. It is possible to reduce the accuracy of evaluation because of lose information. Unsupervised learning is a potential method which may solve this problem because we use all the information for the evaluation process.
This paper is aimed for evaluating different evaluating knowledge representation learning methods by clustering algorithms and classification algorithms.

This paper is organized as follows: the first section reviews the latest research about evaluation protocol like link prediction task. We introduce the two metrics of link prediction task: mean rank and hits@n. 
\\\\
Then we shortly represent the data extracted from patient electronic health records (EHR) and the knowledge representation learning methods we will comparing. In order to identify which set of parameters are more appropriate for each dataset shape being taken into account, we use different combinations of hyper-parameters used along the Knowledge representation learning process. 
\\\\
Evaluation Scenarios including three individual distinct dimensions: (i) the categorization aspect, (ii) the hierarchical aspect, and (iii) the relational aspect. The categorization aspect is to represent how far is the categorization aspect of concepts captured by an embedding model? In other words, we aim to measure the quality of the embedding for concepts via observing their behaviour in categorization tasks. 

To test the accuracy of embedding process, we use two methods to evaluate the embedding process: unsupervised learning and supervised learning. 
\\\\
In first part, we use k-means clustering algorithm to evaluating embedding learning methods and compare the results with link prediction task.
\\\\
In second part, we use a multi-layer perceptron as the supervised learning evaluating method. We training the classifier and test the accuracy of classification process
\\\\
The link prediction task~\cite{2013_Bordes_TransE}
is used to estimate our translating embedding method. The link prediction task is focus on the prediction of missing head entity or tail entity in $(h, r, t)$ and it including two metrics: mean rank and hits@n. In this project, we focus on the part of replace tail entity only.To calculate the mean rank, we replace the real tail entity for each triple (h, r, t) in the test set with all the entities in the dictionary and we can obtain fake triples. Then we calculate the score by the function fr(h,t) in order to get all the potential tail we could expect from the all the fake triples. Through this way, we can get a series of scores and then sort the scores in ascending order. 
% LaTex does NOT understand # only \# (# is a special character)
Next, we adjust those entities in the candidate set for relation r ahead of non- candidate set and keep the order relatively unchanged both in candidate set and non-candidate set.
(I am not really understand this part which copy from : Translating Embeddings for Knowledge Graph Completion with Relation Attention Mechanism by Wei Qian).  
Finally, we record the position of the correct triple tail entity and calculate the mean value of all the correct triples. The smaller the position of real tail, the better transE is.

Another part is hits@n. We also use the process of calculate mean rank. When we find one correct tail in top n result and it will be count once. Then we can obtain the total number of correct tail occur in top n result. Then the hits@n is the total number of count divided by the overall number of test triples.
%Do I need to explain why we choose hits@10 and why we only consider fake tail instead of the average value of head and tail?#


\subsection{Some related work from HEXTRATO paper}

% === TransE ===

(\hl{KDIR}~\cite{2018_HEXTRATO} - {\color{red} PARAPHRASING REQUIRED})
Although TransE is very efficient while achieving predictive performance, it rifts on dealing with certain kinds of relations, such as reflexive, one-to-many, many-to-one, and many-to-many relationships~\cite{2014_Wang_TransH}. Nevertheless, other methods utilise TransE as a base model as part of the first learning steps in order to provide the initial embeddings, aiming to learn better knowledge representations for complicated semantic correlations between knowledge triples -- e.g. by projecting the entity embedding vector into a relation space using relation-specific matrices. Some of these translation-based embedding models are briefly described below.

% === TransE EXTENSIONS ===

(\hl{KDIR}~\cite{2018_HEXTRATO} - {\color{red} PARAPHRASING REQUIRED})
TransH~\cite{2014_Wang_TransH} models relations as hyperplanes together with translation operations on it. TransH overcomes the flaws \ignore{of TransE} regarding to those kinds of relationships that TransE does not perform well, by preserving the mapping properties of relations, and keeping the same model complexity and running time of TransE. Each entity can have distinct distributed representations when involved in different relations, which allows entities to play different roles in different relations. Each relation \emph{r} is represented by a vector $r$ on a hyperplane with $w_r$ as the normal vector. The entity embedding vectors \emph{h} and \emph{t} are first projected to the hyperplane of $w_r$ ($h_{\perp}$ and $t_{\perp}$). The score function is similar to that used in TransE, but using the projected embedding vectors instead (Equation \ref{equation:TransH}).

(\hl{KDIR}~\cite{2018_HEXTRATO} - {\color{red} PARAPHRASING REQUIRED})
\begin{equation}\label{equation:TransH}
f_r(h,t) = \lVert h_{\perp} + r - t_{\perp} \rVert_2^2
\end{equation}

(\hl{KDIR}~\cite{2018_HEXTRATO} - {\color{red} PARAPHRASING REQUIRED})
TransR~\cite{2015_Lin_TransR} and ETransR~\cite{2017_Lin_ETransR} model entity and relation embedding representation into separate distinct vector spaces, bridged by a relation-specific matrix $M_r$ (a $k$-dimensional space for entities and a $m$-dimensional space for relations). These methods are mainly focused on modelling single knowledge in continuous space instead of modelling the semantic relatedness between knowledges. In these models, the entity and relation embedding dimensions are not necessarily identical. In ETransR, however, all the results report $k = m$, which lead us to conclude that: a)  projecting entity embedding vectors into lower dimensional spaces can lose some precious information, and b) using higher dimensional spaces do not necessarily add any further useful information to the embedding model.

(\hl{KDIR}~\cite{2018_HEXTRATO} - {\color{red} PARAPHRASING REQUIRED})
Structured Embedding or SE~\cite{2011_Bordes_SE} and STransE~\cite{2016_Nguyen_STransE} intend to account for relationship asymmetry by using two relation-specific projection matrices for entities \emph{h} and \emph{t}. SE defines the score function by using two projected vectors, so that:

(\hl{KDIR}~\cite{2018_HEXTRATO} - {\color{red} PARAPHRASING REQUIRED})
\begin{equation}\label{equation:SE}
f_r(h, t) = \lVert W_{r,1}h - W_{r,2}t \lVert
\end{equation}


(\hl{KDIR}~\cite{2018_HEXTRATO} - {\color{red} PARAPHRASING REQUIRED})

\noindent 
where $f_r(h, t)$ is large for corrupted triplets (and small otherwise) in some subspace that depends on the relationship \emph{r}. STransE combines SE and TransE by using relation-specific matrices $W_{r,1}$ and $W_{r,2}$ to identify the relation-dependent aspects, and a vector $r$ to capture the relationship between the entities \emph{h} and \emph{t}. In STransE, a score function $f_r(h,t)$ (Equation \ref{equation:STransE}) is used to minimize the margin-based objective function, and performs better than the SE, TransE and other state-of-the-art link prediction models.

(\hl{KDIR}~\cite{2018_HEXTRATO} - {\color{red} PARAPHRASING REQUIRED})
\begin{equation}\label{equation:STransE}
f_r(h,t) = \lVert W_{r,1}h + r - W_{r,2}t \rVert_{l_{1/2}}
\end{equation}

(\hl{KDIR}~\cite{2018_HEXTRATO} - {\color{red} PARAPHRASING REQUIRED})
TransT~\cite{2017_TransT} is a recent attempt to integrate structured information and entity types in order to describe the categories of entities. TransT constructs relation types from entity types and utilises type-based semantic similarity to capture prior distributions of entities and relations. However, it gerenates multiple embedding representations of each entity in different contexts.

(\hl{KDIR}~\cite{2018_HEXTRATO} - {\color{red} PARAPHRASING REQUIRED})
Knowledge embedding methods are commonly evaluated on standard benchmark datasets WN18 and FB15K built with data extracted from Wordnet~\cite{1998_Fellbaum_Wordnet} and Freebase~\cite{2008_Bollacker_Freebase}. Reporting results~\cite{2015_Lin_TransR,2016_Nguyen_STransE}, however, evidence the lack of accuracy when dealing with non-categorised data  available in this traditional benchmark datasets.

(\hl{KDIR}~\cite{2018_HEXTRATO} - {\color{red} PARAPHRASING REQUIRED})
Type-based constraints can support the statistical modelling with latent variable models, by integrating prior knowledge on entity and relation types, significantly improving these models up to about 70\% in link prediction tasks, especially when a low model complexity is enforced~\cite{krompassISWC2015}. 

\
%\subsection{Rewrite the related work from HEXTRATO paper}
% === TransE ===

%(\hl{KDIR}~\cite{2018_HEXTRATO}
%Although TransE is very helpful in achieving predictive performance, it has some limitations when dealing with certain types of relationships, for example reflexive, one-to-many, many-to-one, and many-to-many relationships~\cite{2014_Wang_TransH}.However, other methods use TransE as the base model to provide initial embedding, designed to learn the complex semantics between knowledge triples and to better represent the knowledge - for example, by projecting the entity embedding vector into the relational space using a relation-specific matrix in. The following is a brief example of using a translation-based embedded model.

% === TransE EXTENSIONS ===

%(\hl{KDIR}~\cite{2018_HEXTRATO}
%TransH~\cite{2014_Wang_TransH} transforms the relational model into a hyperplane and its associated translations and maintains the same model complexity and runtime by preserving the mapping properties of the relationship, overcoming the shortcomings of those relationships that TransE does not perform well\ignoring{of TransE }. When different relationships are involved, each entity can have a different distributed representation, which allows entities to play different roles in different relationships. Each relation \emph{r} is represented by a vector $r$ on a hyperplane with $w_r$ as the normal vector. The entity embedding vectors \emph{h} and \emph{t} are first projected to the hyperplane of $w_r$ ($h_{\perp}$ and $t_{\perp}$). The score function is similar to that used in TransE, but using the projected embedding vectors instead (Equation \ref{equation:TransH}).

%(\hl{KDIR}~\cite{2018_HEXTRATO}
%\begin{equation}\label{equation:TransH}
%f_r(h,t) = \lVert h_{\perp} + r - t_{\perp} \rVert_2^2
%\end{equation}
 
%(\hl{KDIR}~\cite{2018_HEXTRATO}
%TransR~\cite{2015_Lin_TransR} and ETransR~\cite{2017_Lin_ETransR} Model entities and relationships are embedded into separate different vector spaces, bridged by a relation-specific matrix $M_r$ (a $k$-dimensional space of the entity and the $m$ -dimensional space of the relationship). These methods focus primarily on modeling individual knowledge in a contiguous space rather than the semantic relevance between modeling knowledge. In these models, the entity and relationship embedding dimensions are not necessarily the same. However, in ETransR, all results report $k =m $, which leads us to the following conclusions: a) Entity embedding entities into low-dimensional spaces may lose some valuable information, and b) use higher Dimensional space does not necessarily add any other useful information to the embedded model.
